CityGaussianV2: Efficient and Geometrically Accurate Reconstruction for Large-Scale Scenes

Recently, 3D Gaussian Splatting (3DGS) has revolutionized radiance field reconstruction, manifesting efficient and high-fidelity novel view synthesis. However, accurately representing surfaces, especially in large and complex scenarios, remains a significant challenge due to the unstructured nature of 3DGS. In this paper, we present CityGaussianV2, a novel approach for large-scale scene reconstruction that addresses critical challenges related to geometric accuracy and efficiency. Building on the favorable generalization capabilities of 2D Gaussian Splatting (2DGS), we address its convergence and scalability issues. Specifically, we implement a decomposed-gradient-based densification and depth regression technique to eliminate blurry artifacts and accelerate convergence. To scale up, we introduce an elongation filter that mitigates Gaussian count explosion caused by 2DGS degeneration. Furthermore, we optimize the CityGaussian pipeline for parallel training, achieving up to 10$\times$ compression, at least 25% savings in training time, and a 50% decrease in memory usage. We also established standard geometry benchmarks under large-scale scenes. Experimental results demonstrate that our method strikes a promising balance between visual quality, geometric accuracy, as well as storage and training costs. The project page is available at https://dekuliutesla.github.io/CityGaussianV2/.

==> sections/0_abstract_arXiv.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.99\textwidth]{figs/teaser.pdf}
\caption{Illustration of the superiority of CityGaussianV2. (a) Our method reconstructs large-scale complex scenes with accurate geometry from multi-view RGB images, restoring intricate structures of woods, buildings, and roads. (b) ``Ours-coarse`` denotes training 2DGS with our optimization algorithm. This strategy accelerates 2DGS reconstruction in terms of both rendering quality (PSNR, SSIM) and geometry accuracy (F1 score).  (c) Our optimized parallel training pipeline reduces the training time and memory by 25\% and 50\% respectively, while achieving better geometric quality. We report mean quality metrics in \textit{GauU-Scene} \citep{xiong2024gauuscene} here, with the best performance in each column highlighted in \textbf{bold}.}
\label{fig: teaser}
\end{figure}

\begin{abstract}
Recently, 3D Gaussian Splatting (3DGS) has revolutionized radiance field reconstruction, manifesting efficient and high-fidelity novel view synthesis. However, accurately representing surfaces, especially in large and complex scenarios, remains a significant challenge due to the unstructured nature of 3DGS. In this paper, we present CityGaussianV2, a novel approach for large-scale scene reconstruction that addresses critical challenges related to geometric accuracy and efficiency. Building on the favorable generalization capabilities of 2D Gaussian Splatting (2DGS), we address its convergence and scalability issues. Specifically, we implement a decomposed-gradient-based densification and depth regression technique to eliminate blurry artifacts and accelerate convergence. To scale up, we introduce an elongation filter that mitigates Gaussian count explosion caused by 2DGS degeneration. Furthermore, we optimize the CityGaussian pipeline for parallel training, achieving up to 10$\times$ compression, at least 25\% savings in training time, and a 50\% decrease in memory usage. We also established standard geometry benchmarks under large-scale scenes. Experimental results demonstrate that our method strikes a promising balance between visual quality, geometric accuracy, as well as storage and training costs. The project page is available at \url{https://dekuliutesla.github.io/CityGaussianV2/}.
\end{abstract}

% key words: neural rendering, novel view synthesis, large-scale scene, radiance field, surfel splatting,  surfel reconstruction

==> sections/4_experiments_rebuttal.tex <==
\section{Geometric evaluation protocols}
\label{sec: eval}
\begin{figure}[t]
\centering
\includegraphics[width=0.99\textwidth]{figs/pipeline-eval.pdf}
\caption{Illustration of the evaluation process.}
\label{fig: pipeline-eval}
\end{figure}

The evaluation protocol for rendering quality is well-established and transferable. We adhere to standard practices by measuring SSIM, PSNR, and LPIPS between renderings and groundtruth. However, there is still no universally accepted protocol for assessing geometric accuracy in large-scale scene reconstruction. Recently, \textit{GauU-Scene} \citep{xiong2024gauuscene} introduced the first benchmark, but its evaluation protocol overlooks boundary effects, leading to unreliable assessments. For instance, as indicated in its own paper \citep{xiong2024gauuscene}, such a protocol significantly underestimates the geometric accuracy of SuGaR, which demonstrates promising performance in mesh visualization. Moreover, \textit{GauU-Scene} does not align the surface points extraction process across methods, leading to unfair comparison. In particular, NeRF-based methods extract points from depth maps, while 3DGS utilizes Gaussian means. To address these issues, we draw lessons from the evaluation protocol of the Tanks and Temple (TnT) dataset \citep{knapitsch2017tanks}, which includes point cloud alignment, resampling, volume-bound cropping, and F1 score measurement. For all the compared methods, we first extract mesh and then sample points from the surface. Though TnT's strategy of sampling vertices and face centers is fast, it would underestimate the effect of mistakenly posing large triangles. Therefore, we sample same number of points evenly on the surface.

To further deal with the challenge of boundary effect, an appropriate estimation of the crop volume is necessary. The core here is to check the visible frequency of each point and estimate a bound that can exclude rarely observed points. For efficiency, we take a workaround that formulates points as Gaussian primitives and checks their visibility using a well-optimized GS rasterizer. As illustrated in \cref{fig: pipeline-eval}, we begin by initializing a 3DGS field with the ground-truth point cloud, then traverse all training views to rasterize and count visible frequency through the output visible mask. If the frequency of $j$-th point $\tau_j$ is below a predefined threshold, it will be excluded. Then we calculate the minimum and maximum height of the remaining points, and project them to the ground plane with ground-truth transformation matrix for alpha shape estimation. Given a scene covering $1.47km^2$ with 958 training views and 31.4 million ground-truth points, this process can be completed within 1 minute if rendered in 1080p on a 40G A100. Compared to the crop volume estimated on all points, ours reduces the error bar length of the F1 score from 0.1 to 0.003, enabling a stable, consistent, and reliable evaluation of the model's actual performance. 

Aside from automatic crop volume estimation, we also downsample the ground-truth point cloud to accelerate the evaluation process under such large-scale scenes. The downsampling voxel size is set to 0.35m. The distance threshold of $\tau$ varies from 0.3m to 0.6m, according to statistics of nearest-neighbor distances in the downsampled ground-truth point clouds. 

\section{Experiments}
\label{sec: 4. experiment}


\subsection{Experimental Setup}
\label{subsec: exp}

\begin{figure}[h]
\centering
\includegraphics[width=0.99\textwidth]{figs/vis_geometry.pdf}
\caption{Qualitative comparison of surface reconstruction quality. Here ``Russian`` and ``Modern`` denote the Russian Building and Modern Building scene of \textit{GauU-Scene}, respectively. And ``Aerial`` denotes aerial view of \textit{MatrixCity}. The messy results of GOF are mainly attributed to the near-ground shell-like mesh. Due to the page limit, we leave further qualitative comparison with GOF and visualization at street view in the Appendix.}
\label{fig: geometry}
\end{figure}

\textbf{Datasets}. We require datasets with accurate ground-truth point clouds. Therefore, we utilize the realistic dataset \textit{GauU-Scene} \citep{xiong2024gauuscene} and the synthetic dataset \textit{MatrixCity} \citep{li2023matrixcity}. From \textit{GauU-Scene}, we selected the Residence, Russian Building, and Modern Building scenes. For \textit{MatrixCity}, we conduct experiments on its aerial view and street view version respectively. Each scene comprises over 4,000 training images and more than 450 test images, presenting significant challenges. These five scenes span areas ranging from 0.3 km$^2$ to 2.7 km$^2$. For aerial views, we follow \cite{kerbl20233d} to downsample the longer side of images to 1,600 pixels. For street views, we retain the original 1,000 × 1,000 resolution. To generate the initial sparse point cloud, we employ COLMAP \citep{schoenberger2016sfm, schoenberger2016mvs} along with the provided poses. Ground-truth point clouds are exclusively utilized for geometry evaluation.

\textbf{Implementation Details}. All experiments included in this paper are conducted on 8 A100 GPUs. We set the gradient scaling factor $\omega$ to 0.9 and the pruning ratio to 0.025. For depth distortion loss, we empirically find it harmful to performance, and thus set its weight to default value 0. The weight for $\mathcal{L}_{\mathrm{Depth}}$ is exponentially decayed from 0.5 to 0.0025 during both the pretraining and fine-tuning stages. $\mathcal{L}_{\mathrm{Normal}}$ is activated after 7,000 iterations in pretraining and from the beginning in the parallel tuning. Besides, we found that the original normal supervision was overly aggressive for complex scene reconstruction. Consequently, the weight for $\mathcal{L}_{\mathrm{Normal}}$ is reduced to 0.0125, one-fourth of its original value. We adhere to the default settings in CityGaussian \citep{liu2024citygaussian} for the learning rate and densification schedule. To be specific, it applies lower learning rates during tuning compared to pertaining, and the street view is trained with a significantly lower learning rate and longer densification interval due to its extreme view sparsity \citep{zhou2024drivinggaussian}. Due to page limitations, additional details, including parameters for block partition and quantization, are provided in the Appendix.

For depth rendering, we utilize median depth for improved geometry accuracy, and for mesh extraction, we employ 2DGS's TSDF-based algorithm with a voxel size of 1m and SDF truncation of 4m. Additionally, \textit{GauU-Scene} applies depth truncation of 250m, while \textit{MatrixCity} uses 500m.

\textbf{Baselines}. We compare our method against state-of-the-art Gaussian Splatting methods for surface reconstruction, including SuGaR \citep{guedon2024sugar}, 2DGS \citep{huang20242d}, and GOF \citep{yu2024gaussian}. Implicit NeRF-based methods such as NeuS \citep{wang2021neus} and Neuralangelo \citep{li2023neuralangelo} are also included. For a fair comparison, we follow \cite{lin2024vastgaussian, liu2024citygaussian} to double the total iterations; the starting iteration and interval of densification for GS-based or warm-up and annealing iteration of NeRF-based methods are likewise doubled. We observed that GOF's mesh extraction generates an extremely high-resolution mesh exceeding 1G, significantly larger than the meshes produced by the original settings of SuGaR and 2DGS. To ensure fairness, we adjusted the mesh extraction parameters of these methods to align their resolutions. For large-scale scene reconstruction, we utilize CityGaussian \citep{liu2024citygaussian} as a representative, as other concurrent aerial-view-based methods were not open-sourced at the time of submission. For its mesh extraction, we adopt 2DGS's methodology and use median depth for TSDF integration.

\subsection{Comparison with SOTA methods}
\label{subsec: sota}

\begin{table}[t]
  \caption{Comparison with SOTA reconstruction methods. ``NaN`` means no results due to NaN error. ``FAIL`` means the method fails to extract meaningful mesh due to poor convergence. Here P and R denotes precision and recall against ground-truth point cloud, respectively. More detailed rendering metrics are included in the Appendix. }
  \label{tab: sota}
  \begin{center}
  \tabcolsep=0.15cm
  \resizebox{0.99\textwidth}{!}{
  \begin{tabular}{lcccccccccccc}
    \toprule
     & \multicolumn{4}{c} {GauU-Scene} &\multicolumn{4}{c}{MatrixCity-Aerial} & \multicolumn{4}{c}{MatrixCity-Street}\\
     \cmidrule(r){2-5} \cmidrule(r){6-9} \cmidrule(r){10-13} 
    Methods & PSNR$\uparrow$ & P$\uparrow$ & R$\uparrow$ & F1$\uparrow$  & PSNR$\uparrow$ & P$\uparrow$ & R$\uparrow$ & F1$\uparrow$ & PSNR$\uparrow$ & P$\uparrow$ & R$\uparrow$ & F1$\uparrow$ \\
    \midrule
    NeuS &14.46 &FAIL &FAIL &FAIL &16.76 &FAIL &FAIL &FAIL &12.86 &FAIL &FAIL &FAIL \\
    Neuralangelo &NaN &NaN &NaN &NaN &19.22 &0.080 &0.083 &0.081 &15.48 &FAIL &FAIL &FAIL\\
    SuGaR &23.47 &\secondbest 0.570 &0.292 &0.377 &22.41 &0.182 &0.157 &0.169 &19.82 &0.053 &0.111 &0.071 \\
    GOF &22.33 &0.370 &0.390 &0.374 &17.42 &FAIL &FAIL &FAIL &20.32 &0.219 &0.473 &0.300\\
    2DGS &23.93 &0.553 &\secondbest 0.446 &\secondbest0.491 &21.35 &0.207 &0.390 &0.270 &21.50 &\secondbest 0.334 &0.659 &\secondbest0.443 \\
    CityGS &\best24.75 &0.522 &0.405 &0.453 &\best 27.46 &\secondbest 0.362 &\secondbest 0.637 &\secondbest0.462 &\best22.98 &0.283 &\secondbest 0.689 & 0.401 \\
    Ours &\secondbest24.51 &\best 0.576 &\best 0.450 &\best0.501 &\secondbest 27.23 &\best 0.441 &\best 0.752 &\best0.556 &\secondbest22.24 &\best 0.376 &\best 0.759 &\best0.503 \\
    \bottomrule
  \end{tabular}
}\end{center}
\end{table}
\vspace{-.1in}

In this section, we compare CityGaussianV2 with state-of-the-art (SOTA) methods both quantitatively and qualitatively. \cref{tab: sota} report results with no compression. As shown, NeRF-based methods are more prone to failure due to the NaN outputs of the MLP or poor convergence under sparse supervision in large-scale scenes. Besides, these methods generally take over 10 hours for training. In contrast, GS-based methods finish training within several hours, while demonstrating stronger performance and generalization abilities. For \textit{GauU-Scene}, our model significantly outperforms existing geometry-specialized methods in rendering quality. As visually illustrated in \cref{fig: rendering}, our method accurately reconstructs details such as crowded windows and woodlands. Geometrically, our model outperforms 2DGS by 0.01 F1 score. Besides, part (b) of \cref{fig: teaser} shows that even without parallel tuning, our proposed optimization strategy enables our model to achieve significantly better performance in rendering and geometry at both 7K and 30K iterations, while 2DGS struggles to efficiently optimize large and blurry surfels. This validates our superiority in convergence speed. Compared to CityGS, though 0.24 PSNR is sacrificed, our method gains on average 0.05 F1-score (around 11\%) improvement. As validated in \cref{fig: geometry}, the meshes produced by our method are smoother and more complete.

On the challenging \textit{MatrixCity} dataset, we evaluate performance from both aerial and street views. For MatrixCity-Aerial, our method achieves the best surface quality among all algorithms, with the F1 score being twice that of 2DGS and outperforming CityGaussian by a significant margin. Furthermore, GOF fails to complete training or extract meaningful meshes. In the street view, CityGS and geometry-specialized methods like 2DGS significantly underperform our method in geometry. As illustrated in \cref{fig: street} in the Appendix, our method provides qualitatively better reconstructions of road and building surfaces, with rendering quality comparable to CityGS.

Regarding training costs, as indicated in \cref{tab: ablation}, the small version of CityGaussianV2 (ours-s) reduces training time by 25\% and memory usage by over 50\%, while delivering superior geometric performance and on-par rendering quality with CityGS. The tiny version (ours-t) can even halve the training time. These advantages make our method particularly suitable for scenarios with varying quality and immediacy requirements. Results on other scenes are included in \cref{tab: sota-statistics} of Appendix.
 
\subsection{Albation Studies}
\label{subsec: ablations}

\begin{table}[h]
  \caption{Ablation on model components. The experiments are conducted on Residence scene of \textit{GauU-Scene} dataset (\citep{xiong2024gauuscene}). Here we take 2DGS (\citep{huang20242d}) as our baseline. The upper part ablates on pertaining, while the lower part ablates on fine-tuning. \#GS, T, Size, Mem. are the number of Gaussians, total training time with 8 A100, memory, storage cost. \textit{The units are million, minute, Gigabytes, and Gigabytes respectively}. The best performance of each part is in \textbf{bold}.  ``+`` means add components on basis of all components in the above rows. An indented line means that only the module in that line is added, while that of other indented rows are excluded. The \colorbox{gray!20}{gray} row denotes modification that is aborted and not included in the following experiments. }
  \label{tab: ablation}
  \begin{center}
  \resizebox{0.99\textwidth}{!}{
  \begin{tabular}{lllllllccccc}
    \toprule
     & \multicolumn{3}{c} {Rendering Quality} &\multicolumn{3}{c}{Geometric Quality} & \multicolumn{5}{c}{GS Statistics}\\
     \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-12}
    Model & SSIM$\uparrow$ & PSNR$\uparrow$ & LPIPS$\downarrow$ & P$\uparrow$ & R$\uparrow$ & F1$\uparrow$ &\#GS &T &Size &Mem. &FPS \\
    \midrule
    Baseline &0.637 &21.12 &0.401 &0.474 &0.362 &0.410 &9.54 &\textbf{78} &2.26 &20.8 &28.0\\
    + Elongation Filter &0.636 &21.18 &0.401 &0.477 &0.362 &0.411 &\textbf{9.36} &\textbf{78} & 2.26 &20.8 &28.6\\
    + DGD &0.674 &\textbf{22.24} &0.345 &0.480 &0.387 &0.429 &9.51 &84 &\textbf{2.25} &20.7 &30.3\\
    + Depth Regression &\textbf{0.674} &22.22 &\textbf{0.345} &\textbf{0.501} &\textbf{0.390} &\textbf{0.438} &9.67 &89 & 2.29 &25.3 &29.4 \\
    % + Exp. Depth Reg. &\textbf{0.686} &\textbf{22.50} &\textbf{0.331} &0.434 &\textbf{0.377} &0.404 &10.3 &89 & 2.43 \\
    \midrule
    + Parallel Tuning &0.742 &23.50 &\textbf{0.237} &0.538 &0.419 &0.471 &19.3 &195 & 4.57 &31.5 &21.3 \\
    \quad + Trim (Ours-b) &\textbf{0.742} &\textbf{23.57} &0.243 &0.534 &0.430 &0.477 &8.07 &179 & 1.90 &19.0 &31.3\\
    \rowcolor{gray!20} \quad + Prune &0.738 &23.46 &0.246 &0.538 &0.420 &0.472 &10.3 &168 & 1.90 &24.3 &30.3 \\
    + SH Degree=2 &0.742 &23.49 &0.245 &\textbf{0.540} &\textbf{0.423} &\textbf{0.474} &8.06 &176 & 1.29 &14.2 &34.5 \\
    + VQ (Ours-s) &0.740 &23.46 &0.248 &0.530 &0.414 &0.465 &8.06 &181 & 0.44 &14.2 &34.5\\
    + 7k pretrain (Ours-t) &0.721 &23.17 &0.281 &0.517 &0.416 &0.461 &\textbf{5.31} & \textbf{115} & \textbf{0.29} &\textbf{11.5} &\textbf{41.7}\\
    \rowcolor{gray!20} + partition of 2DGS &0.704 &22.68 &0.296 &0.508 &0.414 &0.456 &4.71 &112 &0.25 &11.3 &43.5 \\
    \midrule
    CityGaussian &0.727 &23.17 &0.266 &0.519 &0.402 &0.453 &8.05 &235 &0.44 &31.5 &66.7 \\
    \bottomrule
  \end{tabular}
}\end{center}
\end{table}

In this section, we ablate each component of our model design. The upper part of \cref{tab: ablation} focuses on the optimization mechanism. As shown, restricting the densification of highly elongated Gaussians has negligible impact on \textbf{pretraining} performance. However, as illustrated in \cref{fig: explosion}, this strategy is essential for preventing Gaussian count explosion during the \textbf{fine-tuning} stage. Additionally, \cref{tab: ablation} demonstrates that our Decomposed Densification Gradient (DGD) strategy significantly accelerates convergence, improving 1.0 PSNR, 0.04 SSIM, and almost 0.02 F1 score. A more detailed analysis of how gradient from different losses affects performance is included in the Appendix. The last two lines in the upper section confirm that depth supervision from Depth-Anything-V2 \citep{yang2024depth} enhances geometric quality considerably.

The lower part of \cref{tab: ablation} examines our pipeline design. With parallel tuning, both rendering and geometry quality show substantial improvements, validating the success of scaling up. For trimming, we use a more aggressive pruning ratio of 0.1, leading to 50\% storage and memory reduction. The result also underscores the importance of trimming for real-time performance. LightGaussian's \citep{fan2023lightgaussian} pruning strategy, however, falls short in preserving rendering quality. By using an SH degree of 2 from scratch, we further reduce storage and memory usage by over 25\%, with marginal impact on rendering performance or geometry accuracy. And speed is improved by 4.2 FPS. Our contribution-based vectree quantization step takes several minutes for compression, but achieves a 75\% reduction in storage. Additionally, by using the result from 7,000 iterations as a pre-train, the total training time decreases from 3 hours to 2 hours, with the model size shrinking to below 300 MB. This compact model is well-suited for deployment on low-end devices like smartphones or VR headsets. However, replacing the block partition with the one generated from 7,000 iterations of 2DGS results in a considerable drop in both the PSNR and F1 score. This suboptimal outcome underscores the importance of fast convergence for efficient training of tiny models.

\subsection{Discussion}
While our method successfully delivers favorable efficiency and accurate geometry reconstruction for large-scale scenes, we also want to discuss its limitations: Firstly, this paper evaluates on the GauUScene and MatrixCity, which feature compensated or ideally constant lighting conditions. Nevertheless, we trust that the consideration of illumination variance and incorporating techniques like decoupled appearance modeling would be helpful for the model's adaptability. Secondly, for mesh extraction, occlusion and lack of observation hinder reconstruction of some road surfaces and building facades. Additionally, TSDF fusion struggles with thin structures, such as spires (see Appendix, \cref{fig: bad case}). Applying more efficient training strategies and advanced mesh extraction algorithms could address these issues. Thirdly, although our compression strategy significantly enhances rendering speed, it still lags behind CityGS even when sharing similar Gaussian counts. Extensive experiments in \cref{tab: sota-statistics} validate this conclusion. Future work should explore deeper optimizations of rasterizers, such as those proposed by \cite{feng2024flashgs}, or the integration of Level of Detail (LoD) techniques \cite{kerbl2024hierarchical, ren2024octree}.

==> sections/dumped.tex <==
\section{Introduction}
Secondly, while large-scale scene datasets equipped with ground-truth point clouds \citep{xiong2024gauuscene, li2023matrixcity} are available, a reliable and standardized evaluation protocol akin to DTU \citep{jensen2014large} or TnT \citep{knapitsch2017tanks} remains absent. For instance, GigaGS \citep{chen2024gigags} relies solely on qualitative geometric comparisons, while GauU-Scene \citep{xiong2024gauuscene} extracts misaligned surface points across different methods and employs CloudCompare software for evaluation. Besides, the boundary effect in large unbounded scenes is overlooked. Because of rare observations at boundary regions, the geometry estimation is error-prone and unstable in these areas. As a result, the metrics can significantly fluctuate and underestimate actual performance.

In summary, our contributions are four-fold:
\begin{enumerate}
    \item We proposed a novel optimization strategy for 2DGS, including depth regression, Decomposed-Gradient-based Densification (DGD), and Elongation Filter. This mechanism enables fast convergence and successful scaling-up.
    \item With our proposed highly optimized parallel scaling-up pipeline, which not only enables 10$\times$ compression, but also brings at most 50\% training time and over 50\% memory reduction compared to CityGaussian.
    \item We introduce a TnT-style evaluation protocol with a novel crop volume generation strategy. This helps standard and reliable evaluation for large-scale scene surface reconstruction.
    \item To the best of our knowledge, our CityGaussianV2 is among the first to apply the Gaussian radiance field in large-scale surface reconstruction. Experimental results validate our SOTA performance both in quality and training cost.
\end{enumerate}

\section{Experiments}

\begin{table}[t]
  \caption{Comparison with SOTA reconstruction methods. "n/a" here means no results due to OOM or NaN error.}
  \label{tab: sota}
  \begin{center}
  \resizebox{0.99\textwidth}{!}{
  \begin{tabular}{lllllllllllll}
    \toprule
     & \multicolumn{4}{c} {GauU-Scene} &\multicolumn{4}{c}{MatrixCity-Aerial} & \multicolumn{4}{c}{MatrixCity-Street}\\
     \cmidrule(r){2-5} \cmidrule(r){6-9} \cmidrule(r){10-13} 
    Methods & SSIM$\uparrow$ & PSNR$\uparrow$ & LPIPS$\downarrow$ & F1$\uparrow$  & SSIM$\uparrow$ & PSNR$\uparrow$ & LPIPS$\downarrow$ & F1$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & LPIPS$\downarrow$ & F1$\uparrow$ \\
    \midrule
    NeuS & \\
    Neuralangelo &n/a &n/a &n/a &n/a \\
    SuGaR &0.628 &22.72 &0.445 &0.377 &n/a &n/a &n/a & n/a &0.662 &19.82 &0.478 &0.071 \\
    GOF &0.705 &22.33 &0.333 &0.374 &0.374 &17.42 &0.588 &0.018 &0.703 &20.32 &0.440 &0.300\\
    2DGS &0.756 &23.93 &0.232 &\textbf{0.491} &0.632 &21.35 &0.562 & 0.270 &\textbf{0.723} &\textbf{21.50} &\textbf{0.477} &0.441 \\
    Ours-6w &\textbf{0.759} &\textbf{24.25} &\textbf{0.226} &0.486 &\textbf{0.734} &\textbf{24.41} &\textbf{0.342} &\textbf{0.361} &0.717 &21.43 &0.487 &\textbf{0.461} \\
    \midrule
    CityGS &\textbf{0.789} &\textbf{24.75} &\textbf{0.176} &0.449 &\textbf{0.865} &27.46 &0.204 &0.462 &\textbf{0.808} &\textbf{22.98} &\textbf{0.301} & 0.401 \\
    Ours &0.768 &24.67 &0.212 &\textbf{0.490} &0.860 &\textbf{28.17} &\textbf{0.170} &\textbf{0.531} &0.784 &22.19 &0.382 & \textbf{0.524} \\
    \bottomrule
  \end{tabular}
}\end{center}
\end{table}

\begin{table}[h]
  \caption{Ablation on model components. The experiments are conducted on Residence scene of GauU-Scene dataset (\citep{xiong2024gauuscene}). The upper part ablates on pertaining, while the lower part ablates on fine-tuning. \#GS, T, and Size are number of Gaussians, total training time with 8 A100, and storage cost respectively. Here we take 2DGS (\citep{huang20242d}) as our baseline.}
  \label{tab: ablation}
  \begin{center}
  \resizebox{0.99\textwidth}{!}{
  \begin{tabular}{lllllllllll}
    \toprule
     & \multicolumn{3}{c} {Rendering Quality} &\multicolumn{3}{c}{Geometric Quality} & \multicolumn{4}{c}{GS Statistics}\\
     \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-11}
    Model & SSIM$\uparrow$ & PSNR$\uparrow$ & LPIPS$\downarrow$ & P$\uparrow$ & R$\uparrow$ & F1$\uparrow$ &\#GS(M) &T(min) &Size(G) &Mem.(G) \\
    \midrule
    Baseline &0.637 &21.12 &0.401 &0.474 &0.362 &0.410 &9.54 &\textbf{78} &2.26 &20.8\\
    + Elongation Filter &0.636 &21.18 &0.401 &0.477 &0.362 &0.411 &9.56 &\textbf{78} & 2.26 &20.8\\
    + DGD &0.674 &22.24 &0.345 &\textbf{0.480} &0.387 &0.429 &\textbf{9.51} &84 &\textbf{2.25} &20.7\\
    + Depth Regression &\textbf{0.686} &\textbf{22.50} &\textbf{0.331} &0.477 &\textbf{0.394} &\textbf{0.432} &10.3 &89 & 2.43 &25.3 \\
    \midrule
    + Parallel Tuning &0.750 &23.81 &\textbf{0.230} &0.515 &0.423 &0.465 &19.3 &195 & 4.57 &31.5 \\
    + Trimming (Ours-b) &\textbf{0.750} &\textbf{23.85} &0.236 &0.530 &0.426 &0.472 &8.07 &179 & 1.90 &19.0\\
    \rowcolor{gray!20} + Pruning &0.738 &23.46 &0.246 &0.529 &0.410 &0.462 &10.3 &168 & 1.90 &24.3 \\
    + SH Degree=2 &0.750 &23.75 &0.237 &\textbf{0.509} &\textbf{0.426} &\textbf{0.464} &8.06 &176 & 1.29 &14.2 \\
    + VQ (Ours-s) &0.748 &23.71 &0.239 &0.530 &0.414 &0.465 &8.06 &181 & 0.44 &14.2 \\
    + 7k pretrain (Ours-t) &0.725 &23.33 &0.281 &0.507 &0.407 &0.451 &\textbf{5.31} & \textbf{115} & \textbf{0.29} &11.5 \\
    \rowcolor{gray!20} CityGaussian &0.758 &23.75 &0.273 &0.511 &0.390 &0.442 &10.9 &254 &0.60 &31.5 \\
    \bottomrule
  \end{tabular}
}\end{center}
\end{table}

% \begin{table}[h]
%   \caption{Ablation on model components. The experiments are conducted on Residence scene of GauU-Scene dataset \citep{xiong2024gauuscene}. \#GS, T, and Size are number of Gaussians, total training time with 8 A100, and storage cost respectively. Here we take 2DGS \citep{huang20242d} as our baseline.}
%   \label{tab:let-bev}
%   \begin{center}
%   \resizebox{0.99\textwidth}{!}{
%   \begin{tabular}{llllllllll}
%     \toprule
%      & \multicolumn{3}{c} {Rendering Quality} &\multicolumn{3}{c}{Geometric Quality} & \multicolumn{3}{c}{GS Statistics}\\
%      \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10}
%     Model & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & P$\uparrow$ & R$\uparrow$ & F1$\uparrow$ &\#GS(M) &T(min) &Size(G) \\
%     \midrule
%     Baseline &0.636 &21.18 &0.401 &0.442 &0.346 &0.388 &9.56 &\textbf{78} & 2.26\\
%     + DGD &0.674 &22.24 &0.345 &0.443 &0.373 &0.405 &\textbf{9.51} &84 & \textbf{2.25} \\
%     + Exp. Depth Reg. &\textbf{0.686} &\textbf{22.50} &\textbf{0.331} &0.434 &\textbf{0.377} &0.404 &10.3 &89 & 2.43 \\
%     \midrule
%     + Parallel Tuning &0.750 &23.81 &\textbf{0.230} &\textbf{0.504} &0.413 &0.454 &20.5 &195 & 4.85 \\
%     + Trimming (Ours-b) &\textbf{0.750} &\textbf{23.85} &0.236 &0.500 &\textbf{0.416} &\textbf{0.454} &8.13 &179 & 1.92 \\
%     + SH Degree=2 &0.750 &23.75 &0.237 &0.498 &0.416 &0.454 &8.26 &176 & 1.29 \\
%     + VQ ((Ours-s Light) &0.748 &23.71 &0.239 &0.498 &0.416 &0.454 &8.26 &181 & 0.45 \\
%     + 7k pretrain (Ours-t) &0.7246 &23.328 &0.28077 &0.468 &0.408 &0.436 &\textbf{5.36} & \textbf{115} & \textbf{0.29} \\
%     \bottomrule
%   \end{tabular}
% }\end{center}
% \end{table}

\subsection{Comparison with SOTA}
\label{subsec: sota}

As shown in the upper part of \cref{tab: sota}, the GS-based method demonstrates stronger generalization ability. For \textit{GauU-Scene}, our coarse model achieves the best rendering quality while maintaining similar geometry accuracy to 2DGS. Additionally, part (b) of \cref{fig: teaser} illustrates that our proposed optimization strategy allows our model to converge to significantly better performance at both 7K and 30K iterations, regarding rendering and geometry. In contrast, 2DGS gets troubled in efficiently optimizing large and blurring surfels. This superiority becoming more pronounced on MatrixCity-Aerial, where 2DGS lags behind our model by 3 PSNR points and 10 F1 score points. Both SuGaR and GOF fail to complete training or extract meaningful meshes. Notably, the messy mesh produced by GOF in \cref{fig: geometry} results from hulls generated by large blurred Gaussians, as depicted in Fig. S1 of the Appendix. We visualize the meshes of both GOF and our method from an interior perspective in Fig. S1, validating that our approach outperforms GOF in both accuracy and completeness. As shown in \cref{fig: rendering}, the suboptimal rendering quality of GOF and 2DGS suffers from overblurring. We also evaluate performance on urban street scenes, i.e. MatrixCity-Street, where our method achieves comparable quality to 2DGS but with superior geometry. 


In comparing the lower part of \cref{tab: sota}, our CityGaussianV2 demonstrates significant scalability and excels in geometry. As illustrated in \cref{fig: geometry}, the meshes produced by our method are smoother and more complete. For rendering, we achieve rendering quality on par with CityGaussian, which is further supported by \cref{fig: rendering}. On the MatrixCity-Aerial dataset, our model significantly outperforms CityGaussian in PSNR. Furthermore, compared to the original CityGaussian \citep{liu2024citygaussian}, our method incurs much lower training costs. As indicated in \cref{tab: ablation}, the small version of CityGaussianV2 (ours-s) reduces training time by 25\% and memory usage by over 50\%, while delivering superior geometric performance and maintaining comparable rendering quality. The tiny version (ours-t) can even halve the training time. These advantages make our method particularly suitable for scenarios with varying quality and immediacy requirements.

\begin{table}[h]
  \caption{Detailed metrics on \textit{GauU-Scene} datasets (\citep{xiong2024gauuscene}).}
  \label{tab: gauU-sota}
  \tabcolsep=0.125cm
  \begin{center}
  \resizebox{0.99\textwidth}{!}{
  \begin{tabular}{lllllllllllll}
    \toprule
     & \multicolumn{4}{c} {Residence} &\multicolumn{4}{c}{Ruassian Building} & \multicolumn{4}{c}{Modern Building}\\
     \cmidrule(r){2-5} \cmidrule(r){6-9} \cmidrule(r){10-13} 
    Methods & SSIM$\uparrow$ & PSNR$\uparrow$ & LPIPS$\downarrow$ & F1$\uparrow$  & SSIM$\uparrow$ & PSNR$\uparrow$ & LPIPS$\downarrow$ & F1$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & LPIPS$\downarrow$ & F1$\uparrow$ \\
    \midrule
    NeuS &15.16 &0.244 &0.674 &n/a &13.65 &0.202 &0.694 &n/a &14.58 &0.236 &0.694\\
    Neuralangelo &n/a &n/a &n/a &n/a & & & & &n/a &n/a & n/a &n/a \\
    SuGaR &0.546 &21.03 &0.507 &0.384 &0.693 &22.97 &0.386 &0.417 &0.644 &24.15 &0.441 &0.329 \\
    GOF &0.652 &20.68 &0.391 &0.411 &0.713* &21.30* &0.322* &0.330* &0.749 &25.01 &0.286 &0.382 \\
    2DGS & 0.703 &22.24 &0.306 &0.458 &0.788 &23.77 &0.189 &\textbf{0.531} &0.776 &25.77 &0.202 &\textbf{0.485} \\
    Ours-6w &\textbf{0.709} &\textbf{22.66} &\textbf{0.292} &\textbf{0.459} &\textbf{0.790} &\textbf{24.15} &\textbf{0.189} &0.516 &\textbf{0.778} &\textbf{25.95} &\textbf{0.196} &0.483 \\
    \midrule
    CityGS &\textbf{0.763} &\textbf{23.59} &\textbf{0.204} &0.436 &\textbf{0.808} &\textbf{24.37} &\textbf{0.163} &0.451 &\textbf{0.796} &\textbf{26.29} &\textbf{0.160} &0.461\\
    Ours &0.742 &23.57 &0.243 &\textbf{0.463} &0.788 &24.31 &0.193 &\textbf{0.525} &0.774 &26.13 &0.200 &\textbf{0.490} \\
    \bottomrule
  \end{tabular}
}\end{center}
\end{table}

\begin{table}[h]
  \caption{Detailed statistics on GauU-Scene datasets (\citep{xiong2024gauuscene}).}
  \label{tab: gauU-statistics}
  \begin{center}
  \resizebox{0.99\textwidth}{!}{
  \begin{tabular}{lllllllllllll}
    \toprule
     & \multicolumn{4}{c} {Residence} &\multicolumn{4}{c}{Ruassian Building} & \multicolumn{4}{c}{Modern Building}\\
     \cmidrule(r){2-5} \cmidrule(r){6-9} \cmidrule(r){10-13} 
    Methods &\#GS(M) &T(min) &Size(G) &FPS &\#GS(M) &T(min) &Size(G) &FPS &\#GS(M) &T(min) &Size(G) & FPS \\
    \midrule
    NeuS & \\
    Neuralangelo & \\
    SuGAR & \\
    GoF & \\
    Trim2DGS & \\
    CityGS &32.2 & & & &13.0 & & & &17.6 & & & \\
    Ours &8.07 &179 &1.90 & &5.94 & & & &8.39 & & & \\
    \bottomrule
  \end{tabular}
}\end{center}
\end{table}


